Elastic alpha scattering experiments and the alpha-nucleus optical potential at low energies

High precision angular distribution data of ($\alpha$,$\alpha$) elastic scattering are presented for the nuclei $^{89}$Y, $^{92}$Mo, $^{106,110,116}$Cd, $^{112,124}$Sn, and $^{144}$Sm at energies around the Coulomb barrier. Such data with small experimental uncertainties over the full angular range (20-170 degrees) are the indispensable prerequisite for the extraction of local optical potentials and for the determination of the total reaction cross section $\sigma_{\rm{reac}}$. A systematic fitting procedure was applied to the presented experimental scattering data to obtain comprehensive local potential parameter sets which are composed of a real folding potential and an imaginary potential of Woods-Saxon surface type. The obtained potential parameters were used in turn to construct a new systematic $\alpha$-nucleus potential with very few parameters. Although this new potential cannot reproduce the angular distributions with the same small deviations as the local potential, the new potential is able to predict the total reaction cross sections for all cases under study.

==> sm144a_exp.tex <==
  15.023 & 9.9443e-01 & 1.1358e-02    &   81.188 & 8.2501e-01 & 1.1285e-02  &  149.154 & 1.5125e-01 & 1.9187e-03 \\
  16.050 & 1.0003e+00 & 1.1369e-02    &   82.193 & 8.0272e-01 & 8.5563e-03  &  151.106 & 1.4843e-01 & 2.3744e-03 \\
  17.076 & 9.9475e-01 & 1.1447e-02    &   83.197 & 7.8205e-01 & 8.4548e-03  &  153.057 & 1.4558e-01 & 1.7674e-03 \\
  18.103 & 9.9632e-01 & 1.1476e-02    &   84.201 & 7.7795e-01 & 8.4650e-03  &  155.007 & 1.4175e-01 & 1.5249e-03 \\
  19.129 & 1.0040e+00 & 1.1373e-02    &   85.204 & 7.5133e-01 & 8.2115e-03  &  156.957 & 1.4222e-01 & 1.7300e-03 \\
  20.156 & 1.0128e+00 & 1.1000e-02    &   86.207 & 7.3524e-01 & 7.9127e-03  &  158.905 & 1.3723e-01 & 1.5221e-03 \\
  21.182 & 1.0036e+00 & 1.0368e-02    &   87.210 & 7.1104e-01 & 7.7805e-03  &  160.853 & 1.3005e-01 & 1.6623e-03 \\
  22.208 & 9.9883e-01 & 1.0315e-02    &   88.211 & 6.9320e-01 & 7.6758e-03  &  162.123 & 1.2510e-01 & 1.9469e-03 \\
  23.233 & 9.9291e-01 & 1.0266e-02    &   89.213 & 6.6963e-01 & 7.2226e-03  &  162.801 & 1.2879e-01 & 1.6782e-03 \\
  24.259 & 1.0037e+00 & 1.0246e-02    &   90.214 & 6.4842e-01 & 7.2072e-03  &  164.747 & 1.3078e-01 & 1.4544e-03 \\
  25.284 & 9.9131e-01 & 1.0209e-02    &   91.214 & 6.4119e-01 & 7.3793e-03  &  166.694 & 1.3469e-01 & 1.5707e-03 \\
  26.309 & 1.0053e+00 & 1.0339e-02    &   92.214 & 6.2289e-01 & 6.9926e-03  &  168.639 & 1.3041e-01 & 1.5328e-03 \\
  27.334 & 1.0085e+00 & 1.0550e-02    &   93.213 & 5.9840e-01 & 6.8849e-03  &  170.585 & 1.1894e-01 & 1.7970e-03 \\
  28.359 & 1.0027e+00 & 1.0288e-02    &   94.213 & 5.8820e-01 & 6.8378e-03  &  171.852 & 1.2050e-01 & 1.9303e-03 \\
  29.384 & 1.0066e+00 & 1.0497e-02    &   95.211 & 5.7078e-01 & 6.6741e-03  &  172.530 & 1.2304e-01 & 1.9399e-03 \\
  30.408 & 1.0198e+00 & 1.5073e-02    &   96.209 & 5.5617e-01 & 6.3424e-03 \\
  31.432 & 1.0206e+00 & 1.0765e-02    &   97.207 & 5.4371e-01 & 6.3622e-03 \\
  32.456 & 1.0133e+00 & 1.0700e-02    &   98.204 & 5.2301e-01 & 6.2452e-03 \\
  33.480 & 1.0101e+00 & 1.0703e-02    &   99.200 & 5.0597e-01 & 5.7763e-03 \\
  34.503 & 1.0028e+00 & 1.0409e-02    &  100.196 & 4.8451e-01 & 5.8156e-03 \\
  35.526 & 9.9627e-01 & 1.0516e-02    &  101.192 & 4.7642e-01 & 5.1353e-03 \\
  36.549 & 9.9647e-01 & 1.0504e-02    &  102.187 & 4.5164e-01 & 5.0754e-03 \\
  37.571 & 9.8968e-01 & 1.0777e-02    &  103.181 & 4.3703e-01 & 4.8139e-03 \\
  38.593 & 9.7495e-01 & 1.0256e-02    &  104.176 & 4.2290e-01 & 4.7648e-03 \\
  39.615 & 9.6950e-01 & 1.0532e-02    &  105.169 & 4.1079e-01 & 4.6410e-03 \\
  40.637 & 9.6466e-01 & 9.7744e-03    &  106.162 & 3.9585e-01 & 4.4592e-03 \\
  41.658 & 9.7528e-01 & 9.8899e-03    &  107.155 & 3.8909e-01 & 4.3815e-03 \\
  42.679 & 9.7642e-01 & 9.8882e-03    &  108.147 & 3.7559e-01 & 4.2371e-03 \\
  43.700 & 9.8185e-01 & 9.8995e-03    &  109.139 & 3.7004e-01 & 4.1823e-03 \\
  44.720 & 9.9564e-01 & 1.0739e-02    &  110.131 & 3.5743e-01 & 4.0724e-03 \\
  45.740 & 9.9389e-01 & 1.0787e-02    &  111.122 & 3.5313e-01 & 4.4442e-03 \\
  46.760 & 1.0090e+00 & 1.0321e-02    &  112.112 & 3.4082e-01 & 4.1145e-03 \\
  47.779 & 1.0311e+00 & 1.0710e-02    &  113.102 & 3.2933e-01 & 3.8544e-03 \\
  48.798 & 1.0241e+00 & 1.0427e-02    &  114.091 & 3.2274e-01 & 3.8990e-03 \\
  49.816 & 1.0356e+00 & 1.0619e-02    &  115.081 & 3.1234e-01 & 3.7879e-03 \\
  50.834 & 1.0309e+00 & 1.4915e-02    &  116.069 & 3.0205e-01 & 3.6464e-03 \\
  51.852 & 1.0264e+00 & 1.0540e-02    &  117.057 & 2.9361e-01 & 3.5441e-03 \\
  52.870 & 1.0372e+00 & 1.0619e-02    &  118.045 & 2.8855e-01 & 3.4788e-03 \\
  53.887 & 1.0473e+00 & 1.0634e-02    &  119.032 & 2.8037e-01 & 3.4015e-03 \\
  54.904 & 1.0615e+00 & 1.2113e-02    &  120.019 & 2.7391e-01 & 3.3467e-03 \\
  55.920 & 1.0585e+00 & 1.2193e-02    &  121.006 & 2.6823e-01 & 3.0816e-03 \\
  56.936 & 1.0729e+00 & 1.1172e-02    &  121.992 & 2.6231e-01 & 3.3439e-03 \\
  57.951 & 1.0859e+00 & 1.1612e-02    &  122.977 & 2.5435e-01 & 3.2114e-03 \\
  58.966 & 1.0707e+00 & 1.1058e-02    &  123.963 & 2.4514e-01 & 3.1427e-03 \\
  59.981 & 1.0765e+00 & 1.1256e-02    &  124.947 & 2.4257e-01 & 3.0962e-03 \\
  60.995 & 1.0784e+00 & 1.2439e-02    &  125.932 & 2.3291e-01 & 2.9983e-03 \\
  62.009 & 1.0856e+00 & 1.1070e-02    &  126.916 & 2.2770e-01 & 2.9369e-03 \\
  63.023 & 1.0811e+00 & 1.1102e-02    &  127.899 & 2.2438e-01 & 2.8588e-03 \\
  64.036 & 1.0562e+00 & 1.0887e-02    &  128.883 & 2.1325e-01 & 2.7834e-03 \\
  65.048 & 1.0508e+00 & 1.0674e-02    &  129.865 & 2.0998e-01 & 2.7413e-03 \\
  66.060 & 1.0530e+00 & 1.0896e-02    &  130.848 & 2.0899e-01 & 2.4601e-03 \\
  67.072 & 1.0813e+00 & 1.1394e-02    &  131.830 & 2.0525e-01 & 2.8782e-03 \\
  68.083 & 1.0539e+00 & 1.1141e-02    &  132.812 & 1.9583e-01 & 2.7198e-03 \\
  69.094 & 1.0510e+00 & 1.1155e-02    &  133.793 & 1.9263e-01 & 2.7122e-03 \\
  70.105 & 1.0272e+00 & 1.0848e-02    &  134.774 & 1.8840e-01 & 2.6513e-03 \\
  71.114 & 9.9017e-01 & 1.9709e-02    &  135.755 & 1.8559e-01 & 2.6127e-03 \\
  72.124 & 9.5337e-01 & 9.8877e-03    &  136.735 & 1.8482e-01 & 2.6003e-03 \\
  73.133 & 9.7721e-01 & 1.0268e-02    &  137.715 & 1.7488e-01 & 2.3660e-03 \\
  74.141 & 9.3970e-01 & 9.9395e-03    &  138.695 & 1.7477e-01 & 2.4885e-03 \\
  75.150 & 9.0827e-01 & 9.3548e-03    &  139.674 & 1.7163e-01 & 2.4374e-03 \\
  76.157 & 9.0651e-01 & 9.6564e-03    &  140.653 & 1.7070e-01 & 2.4102e-03 \\
  77.164 & 9.4688e-01 & 1.0412e-02    &  141.334 & 1.7327e-01 & 2.5866e-03 \\
  78.171 & 9.0078e-01 & 9.9673e-03    &  143.291 & 1.6624e-01 & 2.6274e-03 \\
  79.177 & 8.8001e-01 & 9.8128e-03    &  145.246 & 1.6039e-01 & 2.0330e-03 \\
  80.183 & 8.7745e-01 & 9.6887e-03    &  147.201 & 1.5589e-01 & 1.9312e-03 \\

